Vertex Ordering Problems in Directed Graph Streams

We consider directed graph algorithms in a streaming setting, focusing on problems concerning orderings of the vertices. This includes such fundamental problems as topological sorting and acyclicity testing. We also study the related problems of finding a minimum feedback arc set (edges whose removal yields an acyclic graph), and finding a sink vertex. We are interested in both adversarially-ordered and randomly-ordered streams. For arbitrary input graphs with edges ordered adversarially, we show that most of these problems have high space complexity, precluding sublinear-space solutions. Some lower bounds also apply when the stream is randomly ordered: e.g., in our most technical result we show that testing acyclicity in the $p$-pass random-order model requires roughly $n^{1+1/p}$ space. For other problems, random ordering can make a dramatic difference: e.g., it is possible to find a sink in an acyclic tournament in the one-pass random-order model using polylog$(n)$ space whereas under adversarial ordering roughly $n^{1/p}$ space is necessary and sufficient given $\Theta(p)$ passes. We also design sublinear algorithms for the feedback arc set problem in tournament graphs; for random graphs; and for randomly ordered streams. In some cases, we give lower bounds establishing that our algorithms are essentially space-optimal. Together, our results complement the much maturer body of work on algorithms for undirected graph streams.

==> 5-rank-brief.tex <==
\section{Rank Aggregation} \label{sec:rank-aggr-brief}

Recall the \rank problem and the distance $d$ between permutations, defined in \Cref{sec:prelim}. Note that \rank is equivalent to finding the median of a set of $k$ points under this distance function, which can be shown to be metric. It follows that picking a random ordering from the $k$ input orderings provides a $2$-approximation for \rank.

In \Cref{sec:rank-aggr}, we describe a streaming algorithm for \rank designed along very similar lines to the algorithm in Section~\ref{sec:fast-one-pass}, thereby establishing the following result.

\begin{theorem} \label{thm:rank-aggr}
  There is a one-pass algorithm for \rank that uses $O(\eps^{-2} n \log^2 n)$ space, returns a $(1+\eps)$-approximation with probability $\ge\frac23$, but uses exponential post-processing time.
\end{theorem}


==> 6-conclusion.tex <==
%!TEX root = main.tex

% \section{Conclusion}

% Some open questions: Testing acyclicity in $p$ passes? One pass requires $\Omega(n^2)$ space.


==> 90-old-abstract.tex <==
%!TEX root = main.tex

\begin{abstract}
  We consider {\em directed} graph algorithms in a data streaming setting, focusing on problems concerning orderings of the vertices. This includes such fundamental problems as topologically sorting an input DAG and checking whether the input is in fact a DAG. We also study the related problems of finding a minimum feedback arc set, i.e., the minimum number of edges whose removal yields an acyclic graph, and the problem of finding a sink in a graph. We are interested in  understanding the complexity of these problems in both the settings when the stream is adversarially ordered and when it randomly ordered.
  
  When the input graph can be arbitrary and the edge arrival order is adversarial, we show that most of these problems have high space complexity, precluding sublinear-space solutions in the worst case. Some of these bounds also apply when the stream is randomly ordered: e.g., in our most technical result we show that testing whether a graph is a DAG in the $p$-pass random order model requires roughly $n^{1+1/p}$ space. However, for other problems, random ordering can make a dramatic difference: e.g., it is possible to find a sink in an acyclic tournament in the one pass random order model while only using $\polylog(n)$ space whereas roughly $n^{1/p}$ space is necessary and sufficient given $\Theta(p)$ passes when the edges are adversarially ordered. We also design sublinear algorithms the feedback arc set problem in tournament graphs; for random graphs; and for randomly ordered streams. In some cases, we give lower bounds establishing that our algorithms are essentially space-optimal. Together, our results complement the much maturer body of work on algorithms for {\em undirected} graph streams. 
\end{abstract}

